Solving the TTC 2011 Reengineering Case with Edapt

This paper gives an overview of the Edapt solution to the reengineering case of the Transformation Tool Contest 2011.

==> eptcsdata.tex <==
\providecommand{\firstpage}{149}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.14}{10.4204/EPTCS.74.14}}
\pdfoutput=1

